Electric vehicle charging during the day or at night: a perspective on carbon emissions

We propose an emission-oriented charging scheme to evaluate the emissions of electric vehicle (EV) charging from the electricity sector at the region of Electric Reliability Council of Texas (ERCOT). We investigate both day- and night-charging scenarios combined with realistic system load demand under the emission-oriented vs direct charging schemes. Our emission-oriented charging scheme reduces carbon emissions in the day by 13.8% on average. We also find that emission-oriented charging results in a significant CO2 reduction in 30% of the days in a year compared with direct charging. Apart from offering a flat rebate for EV owners, our analysis reveals that certain policy incentives (e.g. pricing) regarding EV charging should be taken into account in order to reflect the benefits of emissions reduction that haven't been incorporated in the current market of electricity transactions.

==> settings.tex <==
% input encoding
\usepackage[utf8]{inputenc}

% package to load content directly from beamer slides
\usepackage[noxcolor]{beamerarticle}

% package from the American Mathematical Society
\usepackage{amsmath}
\usepackage{amssymb}

% package for the multicolumn environment
\usepackage{multicol}

% package for the English language
\usepackage[english]{babel}

% package for graphics
% the formats png, pdf, jpg are permitted
\usepackage{graphicx}

% default graphics path
% \graphicspath{{./logos/}}
\graphicspath{{}}

% Standardpfad für TikZ-Rohdaten
\newcommand{\tikzpath}{./rawdata/}
% Standardendung für TikZ-Rohdaten
\newcommand{\tikzext}{.dat}

% package to allow for dots in filenames
\usepackage{grffile}

% package for subfigures in one figure
\usepackage[caption=false]{subfig}

% define labeling environment
\makeatletter
\newenvironment{labeling}[2][]{%
  \def\sc@septext{#1}%
  \list{}{\settowidth{\labelwidth}{{%
        #2%
          \sc@septext%
      }}%
    \leftmargin\labelwidth \advance\leftmargin by \labelsep
    \let\makelabel\labelinglabel
  }%
}{%
  \endlist
}
\newcommand\labelinglabel[1]{%
  #1\hfil
    \sc@septext%
}
\makeatother

% package for the drawing of figures
\usepackage{tikz}
% library for coordinate calculations
\usetikzlibrary{calc}
% set the default arrow tip
\tikzset{>=latex}
% library for shapes, e.g. ellipse
\usetikzlibrary{shapes}

% package for 3D plots in TikZ
\usepackage{tikz-3dplot}

% package for electrical circuit diagrams
\usepackage[european,americaninductors,straightlabels]{circuitikz}

% package for plotting with TikZ
\usepackage{pgfplots}
% always use the newest version
\pgfplotsset{compat=newest}
% define the style of the connection of two lines
\pgfplotsset{every axis/.append style={line join=bevel}}
% set the default style template
\pgfplotsset{
	every axis/.style={
		width=0.8\textwidth,
		height=0.5\textwidth,
		max space between ticks=50,
	}
}
% align legend entries to the left
\pgfplotsset{legend cell align=left}
% draw a main grid
\pgfplotsset{xmajorgrids}
\pgfplotsset{ymajorgrids}
% set the number of small tickmarks between two main ticks
%\pgfplotsset{minor x tick num={3}}
%\pgfplotsset{minor y tick num={3}}
% draw a finer grid
%\pgfplotsset{xminorgrids}
%\pgfplotsset{yminorgrids}
% scale only the axis
\pgfplotsset{scale only axis}
% define colors like in MATLAB
\definecolor{matlab1}{rgb}{0,0,1}
\definecolor{matlab2}{rgb}{0,0.5,0}
\definecolor{matlab3}{rgb}{1,0,0}
\definecolor{matlab4}{rgb}{0,0.75,0.75}
\definecolor{matlab5}{rgb}{0.75,0,0.75}
\definecolor{matlab6}{rgb}{0.75,0.75,0}
\definecolor{matlab7}{rgb}{0.25,0.25,0.25}
% define a color cycle list like in MATLAB
\pgfplotscreateplotcyclelist{matlab}{
	{matlab1,solid},
	{matlab2,dashed},
	{matlab3,dashdotted},
	{matlab4,dotted},
	{matlab5,densely dashed},
	{matlab6,densely dashdotted},
	{matlab7,densely dotted}% this prevents an error
}
% use the defined color cycle list as default
\pgfplotsset{cycle list name=matlab}
% use the standard color cycle list as default
%\pgfplotsset{cycle list name=color list}
% use a grayscale color cycle list as default
%\pgfplotsset{cycle list name=linestyles}
% set a line width of 1pt
\pgfplotsset{every axis plot/.append style={line width=1pt}}
% use a comma as a dot separator for german plots
\addto\extrasngerman{\pgfplotsset{/pgf/number format/.cd,set decimal separator={{{,}}}}}
% use a half space as the 1000 separator
\pgfplotsset{/pgf/number format/.cd,1000 sep={\,}}
% neue Positionen für Legenden anlegen
\pgfplotsset{/pgfplots/legend pos/north/.style={/pgfplots/legend style={at={(0.50,0.97)},anchor=north}}}
\pgfplotsset{/pgfplots/legend pos/south/.style={/pgfplots/legend style={at={(0.50,0.03)},anchor=south}}}
\pgfplotsset{/pgfplots/legend pos/east/.style={/pgfplots/legend style={at={(0.97,0.50)},anchor=east}}}
\pgfplotsset{/pgfplots/legend pos/west/.style={/pgfplots/legend style={at={(0.03,0.50)},anchor=west}}}
\pgfplotsset{/pgfplots/legend pos/outer north/.style={/pgfplots/legend style={at={(0.50,1.03)},anchor=south}}}

% use the automatic externalization framework of TikZ
\ifpdf
	\usepgfplotslibrary{external}
	%\tikzexternalize
	\tikzsetexternalprefix{external_figs/}
%	\newcommand{\tikzsetnextfilename}[1]{\relax}	
\fi

% package for SI units
\usepackage[binary-units]{siunitx}
% options
% real fractions
\sisetup{per-mode=fraction,mode=math}
% decimal marker in dependence from the language
\addto\extrasngerman{\sisetup{output-decimal-marker={,}}}
\addto\extrasenglish{\sisetup{output-decimal-marker={.}}}
% range phrase in dependence from the language
\addto\extrasngerman{\sisetup{range-phrase={ bis~}}} 
\addto\extrasenglish{\sisetup{range-phrase={ to~}}}

%\definecolor{BoxCol}{rgb}{0.9,0.9,0.9}
% uncomment for grey background to \section boxes 
% for use with default option boxedsections

%\definecolor{BoxCol}{rgb}{0.9,0.9,1}
% uncomment for light blue background to \section boxes 
% for use with default option boxedsections

%\definecolor{SectionCol}{rgb}{0,0,0.5}
% uncomment for dark blue \section text 

% define new mathematical functions
\DeclareMathOperator{\arcosh}{arcosh}

% differential operator (small upright d)
\newcommand*{\diff}{\mathop{}\!\mathrm{d}}

% redefine the exponential function
\DeclareMathOperator{\e}{e}
\renewcommand{\exp}[1]{\e^{#1}}

% write indices upright (in Roman)
\newcommand{\ind}[1]{\mathrm{#1}}

% a period in a math environment
\newcommand{\period}{\,\text{.}}
% a comma in a math environment
\newcommand{\comma}{\,\text{,}}

% magnitude or absolute value
\newcommand{\abs}[1]{\left| #1 \right|}

% mean value or average value
\newcommand{\mean}[1]{\left\langle #1 \right\rangle}

% package for nice fractions in the text mode
\usepackage{xfrac}

% package for better quotes
\usepackage{csquotes}

% % BibLaTeX package for citations
% \usepackage[%
% % 	style=ieee,%				format as used at the IEEE
% % 	backend=biber,% bibtex			suppress warning
%     backend=biber
% ]{biblatex}

% % database of references
% \addbibresource{evChargeRef.bib}

\usepackage{natbib}

% package for an intelligent space character
\usepackage{xspace}

% abbrevations
\newcommand{\eg}{e.\,g.\xspace}
\newcommand{\ie}{i.\,e.\xspace}

% nicer tables
\usepackage{booktabs}
% \usepackage{hyperref}
% package to insert QR (quick-response) codes
\usepackage[]{qrcode}

